Robust Functional Principal Component Analysis for Non-Euclidean Random Objects

Functional data analysis offers a diverse toolkit of statistical methods tailored for analyzing samples of real-valued random functions. Recently, samples of time-varying random objects, such as time-varying networks, have been increasingly encountered in modern data analysis. These data structures represent elements within general metric spaces that lack local or global linear structures, rendering traditional functional data analysis methods inapplicable. Moreover, the existing methodology for time-varying random objects does not work well in the presence of outlying objects. In this paper, we propose a robust method for analysing time-varying random objects. Our method employs pointwise Fr\'{e}chet medians and then constructs pointwise distance trajectories between the individual time courses and the sample Fr\'{e}chet medians. This representation effectively transforms time-varying objects into functional data. A novel robust approach to functional principal component analysis based on a Winsorized U-statistic estimator of the covariance structure is introduced. The proposed robust analysis of these distance trajectories is able to identify key features of time-varying objects and is useful for downstream analysis. To illustrate the efficacy of our approach, numerical studies focusing on dynamic networks are conducted. The results indicate that the proposed method exhibits good all-round performance and surpasses the existing approach in terms of robustness, showcasing its superior performance in handling time-varying objects data.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
